Frequency Domain Identification of Multirate Systems: A Lifted Local Polynomial Modeling Approach

Frequency-domain representations of multirate systems are essential for controller design and performance evaluation of multirate systems and sampled-data control. The aim of this paper is to develop a time-efficient closed-loop identification approach for multirate systems in the frequency-domain. The developed method utilizes local polynomial modeling for lifted representations of LPTV systems, which enables direct identification of closed-loop multirate systems in a single identification experiment. Unlike LTI identification techniques, the developed method does not suffer from bias due to ignored LPTV dynamics. The developed approach is demonstrated on a multirate example, resulting in accurate and fast identification in the frequency domain.

==> LPMLPTVFRF.tex <==
\section{Identification of Time-Invariant Representations of LPTV Systems Using LPM}
\label{sec:MRLPM}
In this section, the method to identify time-invariant representations of LPTV systems in a single experiment is described. First, time-invariant representations for LPTV systems are described, which are used to represent LPTV systems as LTI. Second, LPM is presented, which is used to identify the time-invariant representations. 
\subsection{Time-Invariant Representations of LPTV systems}
\label{sec:timeInvariantRep}
In this paper, two classes of time-invariant representations of LPTV systems are considered, namely the time-lifted and frequency-lifted reformulation. \par
First, the time-lifted reformulation gathers the values of a signal of one period into a larger signal, i.e., the time-lifted signal. The time-lifted representation of LPTV systems, which is a $\fac\times\fac$ LTI system, then relates time-lifted input signals to time-lifted output signals \cite{Bittanti2000}. Define a time-lifted signal as \cite{Ohnishi2021}
\begin{equation}
	\begin{aligned}
	\underline{\nu}\left[ l \right]  &=\lift\nu_h\left[ \dt\right] \\&
	=\begin{bmatrix}
		\nu_h\left[ l\fac\right]  & \nu_h\left[ l\fac+1\right] &\ldots&\nu_h\left[ l\fac+\fac-1\right] 
	\end{bmatrix}^\top \in \mathbb{R}^{\fac}
\end{aligned}
\end{equation}
Now, the time-lifted system $\underline{P}=\lift\ph\lift^{-1}: \; \underline{u}\mapsto\underline{y}$ relates time-lifted inputs to outputs and is LTI \cite{Bittanti2000}. For time-invariant systems, the lifted transfer function is given in \lemmaRef{lemma:timelift}.
\begin{lemma}
	\label{lemma:timelift}
	(Time-lifted transfer function \cite{Bittanti2000}) The time-lifted FRF of an LPTV system over \fac samples is
	\begin{equation}
		\begin{aligned}
			&\underline{P}(\expjwL)= \\
			&\left[\begin{array}{cccccc}
				P^{(0)}(w) & w^{-1} P^{(\fac-1)}(w)  & \cdots & w^{-1} P^{(1)}(w) \\
				P^{(1)}(w) & P^{(0)}(w) & \cdots & w^{-1} P^{(2)}(w) \\
				P^{(2)}(w) & P^{(1)}(w) & \cdots & w^{-1} P^{(3)}(w) \\
				\vdots & \vdots & \ddots & \vdots \\
				P^{(\fac-1)}(w) & P^{(\fac-2)}(w) & \cdots & P^{(0)}(w)
			\end{array}\right] ,
		\end{aligned}
	\end{equation}
	with $w=\expjwL$ and
	\begin{equation}
		\label{eq:Gsigma}
		P^{(\sigma)}(\expjwL) = \frac{{\expjwL}^{\frac{\sigma}{\fac}}}{\fac}\sum_{k=0}^{\fac-1}\ph(e^{j\omega \frac{h_h}{\fac}}\phi^k)\phi^{k\sigma},
	\end{equation}
	with $\phi=e^{\frac{2 \pi j}{F}}$. The inverse relationship for LTI systems is given by
	\begin{equation}
		\label{eq:inverseTimeLift}
		\ph(\expjwH) = \sum_{f=0}^{\fac-1}P^{(\sigma)}\left(e^{j\omega\hl\fac}\right) e^{-\sigma j\omega\hh}.
	\end{equation}
\end{lemma}
\begin{proof}
	See \cite[Section~6.2.1]{Bittanti2009}.
\end{proof}
\alert{add text: From \eqref{eq:Gsigma}, one can conclude that for LTI systems, frequencies are mixed in the time-lifted reformulation????} \par
The second time-invariant representation considered is the frequency-lifted reformulation, which is directly set in the frequency-domain. Consider a signal $\nu_h\left[ \dt\right] $, with discrete-time Fourier transform $N_h(\expjwH)$, define the frequency-lifted vector $\tilde{N}(\expjwH)$
\begin{equation}
	\label{eq:freqLiftSignal}
	\tilde{N}(\expjwH)=\left[\begin{array}{c}
		N_h(\expjwH) \\
		N_h(\expjwH \phi) \\
		N_h\left(\expjwH \phi^{2}\right) \\
		\vdots \\
		N_h\left(\expjwH \phi^{\fac-1}\right)
	\end{array}\right],
\end{equation}
which shows that $i$'th element of the frequency-lifted vector is the original discrete-time Fourier transform, frequency-shifted with $\phi^{i-1}$. For the components $i>1$, this results in signals that are the possibly aliased or imaged versions of the original signal $N_h(\expjwH)$. The relationship between the Fourier transform of the time-domain lifted signal $\underline{N}_l(\expjwL)$ is
\begin{equation}
	\tilde{N}_h(\expjwH) = M_h(\expjwH)\underline{N}_l(\expjwL),
\end{equation}
where
\begin{equation}
	\label{eq:M}
	\resizebox{.87 \linewidth}{!} {$
		\begin{aligned}
			&M_h(\expjwH)= \\
			&\left[\begin{array}{cccc}
				I & z^{-1} & \cdots & e^{\left( -\fac+1\right)\omega\hh } \\
				I & (z \phi)^{-1} & \cdots & (z \phi)^{-\fac+1} \\
				\vdots & \vdots & \cdots & \vdots \\
				I & \left(z \phi^{\fac-1}\right)^{-1} & \cdots & \left(z \phi^{\fac-1}\right)^{-\fac+1}
			\end{array}\right], \end{aligned}$}
\end{equation}
with $z=\expjwH$. Transfer functions of frequency-lifted systems, e.g., transfer function $\tilde{P}(\expjwH): \;\tilde{U}(\expjwH) \mapsto \tilde{Y}(\expjwH)$, are calculated by exploiting the previous result, and can be seen in \lemmaRef{lemma:freqlift}.
\begin{lemma}
	\label{lemma:freqlift} 
	(Frequency-lifted transfer functions \cite{Bittanti2000}) The frequency-lifted transfer function $\tilde{P}(\expjwH)$ is given by
	\begin{equation}
		\tilde{P}(\expjwH) = M(\expjwH)\underline{P}(\expjwL)M(\expjwH)^{-1}
	\end{equation}
For LTI systems, this reduces to
	\begin{equation}
		\label{eq:LTIfLift}
		\begin{split}
			\tilde{\ph}(\expjwH)_{\left[ q+1,p+1\right] } &= \ph(\expjwH\phi^p)\frac{1}{\fac}\sum_{f=0}^{\fac-1}\phi^{f\left( p-q\right) }, \\
			\to 	\tilde{\ph}(\expjwH) &= \operatorname{diag}\left\{\ph(\expjwH\phi^p)\right\},
		\end{split}
	\end{equation}
	having inverse relationship
	\begin{equation}
		\label{eq:inversefLiftSimplified}
		\ph(\expjwH) =\tilde{\ph}(\expjwH\phi^{-p})_{\left[ p+1,p+1\right] }.
	\end{equation}
\end{lemma}
\begin{proof}
	See \cite[Section~6.4.1]{Bittanti2009}.
\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Local Polynomial Modeling}
\label{sec:LPM}
\begin{figure}[tb]
	\centering\includegraphics{pdf/LPMSetup.pdf}
	\caption{Linear system with known input $w$, output $z$ and output noise $v$ considered in LPM.}
	\label{fig:LPMSetup}
\end{figure}
The key idea behind local polynomial modeling is that frequency responses are a smooth function of the frequency. First, consider the open-loop multivariable $\nout\times\nin$ system in \figRef{fig:LPMSetup} and write the DFT of the output of the system as
\begin{equation}
	\label{eq:LPMoutput}
	Z(\fline) = G(\expjwk)W(\fline) + V(\fline) + T(\expjwk) \in \mathbb{C}^{\nout},
\end{equation}
with system $G(\expjwk) \in\mathbb{C}^{\nout\times\nin}$, noise contribution $V(\fline) \in\mathbb{C}^{\nout}$ and transient contribution $T(\expjwk) \in\mathbb{C}^{\nout}$, combining both the noise and system transient. A local window \window can be taken around it in the frequency domain, ranging from $-\windowSize$ to \windowSize
\begin{equation}
	Z(\fline+\window) = G(\expjwkr)W(\fline+\window) + V(\fline+\window) + T(\expjwkr).
\end{equation}
The local models $G(\expjwkr)$ and $T(\expjwkr)$ are parameterized using polynomials, i.e.,
\begin{equation}
	\label{eq:polynomialModels}
	\begin{split}
		G(\expjwkr) &= \ph(\expjwk) + \sum_{s=1}^{R}g_s(\fline)r^s, \\
		T(\expjwkr) &= T(\expjwk) + \sum_{s=1}^{R}t_s(\fline)r^s,
	\end{split}
\end{equation}
with polynomials $g_s(\fline) \in\mathbb{C}^{\nout\times\nin}$ and $t_s(\fline)\in\mathbb{C}^{\nout}$
Using these parameterizations, the output of the system can be rewritten as
\begin{equation}
	\label{eq:windowedOutput}
	\begin{split}
		Z(\fline+\window) &= \left( G(\expjwk) + \sum_{s=1}^{R}g_s(\fline)r^s\right) W(\fline+\window) \\
		&+ T(\expjwk) + \sum_{s=1}^{R}t_s(\fline)r^s + V(\fline+\window) \\
		&= \theta K(\fline+\window) + V(\fline+\window),
	\end{split}
\end{equation}
with $\theta \in \mathbb{C}^{\nout \times \left( R+1\right)\left(\nin+1\right)}$ the matrix of unknown parameters
\begin{equation}
	\resizebox{.88 \linewidth}{!} {$
		\begin{aligned}
			&\theta = \\
			&\begin{bmatrix}G(\expjwk) & g_1(\fline) & \ldots & g_R(\fline) & T(\expjwk) & t_1(\fline) & \ldots & t_R(\fline)
			\end{bmatrix},
		\end{aligned} $}
\end{equation}
and the input data vector $K(\fline+\window)\in\mathbb{C}^{\left( R+1\right)\left(\nin+1\right)\times 1 }$, i.e.,
\begin{equation}
	\begin{aligned}
		K(\fline+\window) = \begin{bmatrix}
			K_1(\window)\otimes W(\fline+\window) \\
			K_1(\window)
		\end{bmatrix} && \text{with } 	K_1 = \begin{bmatrix}
			1 \\ r \\ \vdots \\ r^R
		\end{bmatrix}.
	\end{aligned}
\end{equation}
Collecting the input-output data in \eqref{eq:windowedOutput} for the window \window results in
\begin{equation}
	\label{eq:gatheredWindowedOutput}
	Z_n = \theta K_n+V_n,
\end{equation}
with $X_n = \begin{bmatrix}X(\fline-\windowSize) & \ldots & X(\fline+\windowSize)\end{bmatrix}$. The least-squares optimum to the overdetermined set of equations in \eqref{eq:gatheredWindowedOutput} is equal to
\begin{equation}
	\hat{\theta} = Z_nK_n^H\left(K_nK_n^H \right) ^{-1},
\end{equation}
which is used to approximate the system \ph as
\begin{equation}
	\begin{split}
		\hat{G}(\expjwk) = \hat{\theta}\begin{bmatrix}
			I_{\nin} \\
			0 \\
			\vdots \\
			0
		\end{bmatrix}, 
	\end{split}
\end{equation}
resulting in a local polynomial estimate of the frequency response function. 
\begin{remark}
	Since DFT lines $\fline-\windowSize,\ldots,\fline+\windowSize$ are used for estimating $\hat{G}(\expjwk)$, it means that $\hat{G}(\expjwk)$ is correlated with $\hat{G}(\expjwkr)$ for $\window = -2\windowSize,\ldots,2\windowSize$. This explains why more parameters ($\nout\times(R+1)(\nin+1)$) are able to be identified than the number of measurements \nout.
\end{remark}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{iets over LPM applied to lifted LPTV?}

\alert{PROOF over error naar interpolation+noise?}

==> MRFRF.tex <==
%\section{Multirate Frequency Response Functions}
\label{sec:PFG}
In this section, the method to identify the PFG of a multirate system is presented. First, an alternative description of the PFG is given, that does not require the input to be in the limited signal spaces $\mathcal{W}_P$ or $\mathcal{W}_R$. Second, the method is presented that identifies the plant \ph, which is needed to calculate the alternative definition of the PFG, using the identified time-invariant representation of LPTV systems discussed in \secRef{sec:MRLPM}.
\subsection{Alternative Description of the PFG}
The PFG calculation in \defRef{def:PFG} is time-consuming to identify since the signal space $\mathcal{W}_P$ is limited severely. Therefore, an alternative description of the PFG is given in \lemmaRef{lemma:altPFG}.
\begin{lemma}
	\label{lemma:altPFG}
	(Alternative definition of the PFG \cite{Oomen2007}) The PFG $\mathcal{P}\left(\expjwH\right)$ is given by
	\begin{equation}
		\mathcal{P}\left(\expjwH\right)=\sqrt{\bar{\lambda}\left(\sum_{f=0}^{F-1}\left\|c_{f}\left(\omega_{k}\right)\right\|^{2}\right)},
	\end{equation}
	with
	\begin{equation}
		c_{f}\left(\omega_{k}\right)= \begin{cases}
			\begin{aligned}
				&\ph(\expjwH)\\
				&-\frac{1}{F}\ph(\expjwkH)\izoh\left(\expjwkH\right)\\
				&\cdot Q_{d}\left(\expjwkL\right) \ph\left(\expjwkH\right),
			\end{aligned} & f=0 \\
			\\
			\begin{aligned}
				&-\frac{1}{F} \ph\left(e^{j\hh\left( \omega_k+\left(f/\fac\right) \highfs\right)}\right)\\
				&\cdot\izoh\left(e^{j\hh\left( \omega_k+\left(f/\fac\right) \highfs\right)}\right) \\
				&\cdot Q_{d}\left(\expjwkL\right) \ph\left(\expjwkH\right).
			\end{aligned} & f \neq 0
		\end{cases}
	\end{equation}
\end{lemma}
\begin{proof}
	See \cite{Oomen2007}
\end{proof}
From \lemmaRef{lemma:altPFG} is becomes clear that to calculate the PFG, only a description of the controller \kl, which is assumed to be known, and the plant \ph are necessary. Therefore, the plant \ph is to be identified and will be discussed next.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Recovering the Original System \ph}
\label{sec:liftedPid}
The plant \ph operating in closed-loop is recovered using the identified time-invariant representations discussed in \secRef{sec:MRLPM}. First, the following time-invariant representations of LPTV transfer functions are defined
\begin{align}
	\label{eq:liftedJS}
	\underline{J} = \lift\left(I+\ph \hu \kl \sd\right)^{-1} \ph \lift^{-1} &:& \underline{r}\mapsto\underline{y},\\
	\underline{S} = \lift\left(I+\hu \kl \sd \ph\right)^{-1} \lift^{-1}&:& \underline{r}\mapsto\underline{u},\\
	\tilde{J} = M_{h} \underline{J} M_{h}^{-1}&:& \tilde{r}\mapsto\tilde{y},\\
	\tilde{S} = M_{h} \underline{S} M_{h}^{-1}&:& \tilde{r}\mapsto\tilde{u},
\end{align}
which are identified by using LPM described in \secRef{sec:LPM} by using $w=\underline{\rh}$ or $w=\tilde{\rh}$ and respectively $z=\underline{y}$, $z=\underline{y}$, $z=\tilde{y}$ and $z=\tilde{u}$. 

Second, the time- and frequency-lifted transfer functions $\underline{P}$ and $\tilde{P}$ are recovered by applying \lemmaRef{lemma:liftP}


\begin{lemma}
	\label{lemma:liftP}
	(Calculating $\underline{P}$ or $\tilde{P}$ from transfer functions $\underline{J}$ and $\underline{S}$ or $\tilde{J}$ and $\tilde{S}$) The lifted plant $\underline{P}$ and $\tilde{P}$ are calculated as
	\begin{align}
		\label{eq:liftedP}
		\underline{P}=(\underline{J}) \underline{S}^{-1}, && \tilde{P}=(\tilde{J}) \tilde{S}^{-1}.
	\end{align}
\end{lemma}
\begin{proof}
	Substitute the values for $\underline{J}$, $\underline{S}$, $\tilde{J}$ and $\tilde{S}$ from \eqref{eq:liftedJS} in the right side of \eqref{eq:liftedP}.
\end{proof}
Finally, the inverse lifting procedures, given in \eqref{eq:inverseTimeLift} and \eqref{eq:inversefLiftSimplified}, are applied to estimate \ph, and are repeated here,
\begin{equation}
		\begin{split}
			\ph(\expjwH) &= \sum_{f=0}^{\fac-1}P^{(\sigma)}\left(e^{j\omega\hl\fac}\right) e^{-\sigma j\omega\hh} \\
			\ph(\expjwH) &=\tilde{\ph}(\expjwH\phi^{-p})_{\left[ p+1,p+1\right] }.
		\end{split}
\end{equation}
Resulting in a method that calculates the PFG, using \lemmaRef{lemma:altPFG}, based on identified time- or frequency-lifted representations of LPTV systems.
